Weakly Supervised Volumetric Image Segmentation with Deformed Templates

There are many approaches to weakly-supervised training of networks to segment 2D images. By contrast, existing approaches to segmenting volumetric images rely on full-supervision of a subset of 2D slices of the 3D volume. We propose an approach to volume segmentation that is truly weakly-supervised in the sense that we only need to provide a sparse set of 3D points on the surface of target objects instead of detailed 2D masks. We use the 3D points to deform a 3D template so that it roughly matches the target object outlines and we introduce an architecture that exploits the supervision it provides to train a network to find accurate boundaries. We evaluate our approach on Computed Tomography (CT), Magnetic Resonance Imagery (MRI) and Electron Microscopy (EM) image datasets and show that it substantially reduces the required amount of effort.

==> fig/asm.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}
	\centering
	\includegraphics[height=4.0cm]{fig/asm.png}\\
	(a) Ground truth\hspace{0.5cm} (b) Annotation \hspace{0.7cm}(c) ASM 0-step \hspace{0.75cm}(d) ASM 1-steps\hspace{0.5cm}(e) ASM 2-steps \hspace{0.2cm}
	\vspace{-3mm}
	\caption{\small {\bf Local alignment of atlas to weak annotation} (a) Complete ground truth (b) weak annotation (c) Initial atlas (d) atlas after one ASM step (e) atlas after two ASM steps. }
	\label{fig:asm}
\end{figure*}

==> fig/asm_copy.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}
	\centering
	\includegraphics[height=2.5cm]{fig/atlas_fit.png}\\
	\hspace{0.5cm}  (a) \hspace{2cm} (b)  \hspace{2.5cm}(c) \hspace{2.5cm}(d) \hspace{2.5cm}(e) \hspace{0.5cm}
	\vspace{-2mm}
	\caption{\small {\bf Aligned atlas with a liver for different amount of points ($N$) annotated} (a) Initial sphere atlas (b)  $N = 25$ (c) $N = 125$ (d) $N = 250$ (e) Full annotation which is $N = 3661$ on average for the liver dataset.}
	\label{fig:asm}
\end{figure*}

==> fig/human_results.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[ht]
	\centering 
		\includegraphics[width=0.49\linewidth]{fig/hippocampus_human_results.pdf}
		\includegraphics[width=0.49\linewidth]{fig/liver_human_results.pdf}
		 
	\vspace{-4mm}
	\caption{{\bf Template accuracy} as a function of the number of human or simulated point annotations (N). (a) Hippocampus. (b) Liver.}
	\label{fig:human_results}
\end{figure}

==> fig/manual_anno/manual_anno.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[h]
 
	\centering
	\includegraphics[width=0.32\linewidth]{fig/manual_anno/Groundtruth.png} 
	\includegraphics[width=0.32\linewidth]{fig/manual_anno/FastMarching_a.png}
	\includegraphics[width=0.32\linewidth]{fig/manual_anno/FastMarching_b.png}
	\vspace{-1mm} 
%\vspace{-4mm}
%\includegraphics[height=4cm]{fig/plot2.png} \\
%\hspace{3.8cm}(a) \hspace{4.5cm} (b) \hspace{3cm}  
\caption{\textbf{Use of Fast Marching algorithm from MITK to annotate a liver} (a) Image with ground truth contour (in blue)  (b) Fast Marching algorithm with small $\sigma$  (c) Fast Marching algorithm with large $\sigma$. In both instances, after the initial segmentation, we have to fix false positive and false negative regions.   }}
\label{fig:fast_marching}
\end{figure}

==> fig/mitk_gui.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[ht]
	\centering
	\includegraphics[width=\linewidth]{fig/mitk-plugin-gui.png}
	\caption{\textbf{Annotation GUI} A user can place points by clicking in the 2D image cross sections. A template is then deformed to fit the points and the user can place corrective clicks. The fitting takes less than one second so the process can be done interactively.}
	\label{fig:mitk-gui}
\end{figure}

==> fig/plot1.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[h]
\centering
\includegraphics[width=0.875\linewidth]{fig/plot1.png} \\
\hspace{1.7cm}(a) \hspace{2.5cm} (b) \hspace{3cm} (c) \hspace{1.8cm} 
\vspace{-3mm}
\caption{{\bf Results on the hippocampus dataset.}  (a) {\bf Baseline} (b) \aswnet{} (c) Annotation effort required to achieve $65\%$ and $70\%$ IoU. The blue and red arrows indicate the effort reduction our approach delivers.}
\vspace{-3mm}
\label{fig:plot1}
\end{figure*}

==> fig/plot2.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[h]
\vspace{-3mm}
	\centering
	\includegraphics[width=0.49\linewidth]{fig/plot2a.png} 
	\includegraphics[width=0.49\linewidth]{fig/plot2b.png}
\vspace{-4mm}
%\includegraphics[height=4cm]{fig/plot2.png} \\
%\hspace{3.8cm}(a) \hspace{4.5cm} (b) \hspace{3cm}  
\caption{\textbf{IoU as function of the number of points used (N).} (a) Synaptic Junction dataset.  (b) Liver dataset.  The dashed line denotes fully supervised results.}
\vspace{-5mm}
\label{fig:plot2}
\end{figure}

==> fig/results_many.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[h]
\centering
\includegraphics[height=11cm]{fig/results_many_1.png} \\
\hspace{0.0cm}  (a) \hspace{1.85cm} (b) \hspace{1.8cm} (c) \hspace{2.2cm} (d) \hspace{1.95cm} (e) \hspace{0.45cm}
\caption{Results. (a) A slice from the input volume from top to bottom (b) Ground truth (c) U-Net with full-supervision (d) Baseline (e) \aswnet{}.}
\label{fig:results_more}
\end{figure*} 

==> fig/results_many_2.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[h]  
\centering
\includegraphics[height=14cm]{fig/results_many_2.png} \\
\hspace{0.0cm}  (a) \hspace{1.85cm} (b) \hspace{1.8cm} (c) \hspace{2.2cm} (d) \hspace{1.95cm} (e) \hspace{0.45cm}
\caption{ Results (Cont.). (a) A slice from the input volume from top to bottom (b) Ground truth (c) U-Net with full-supervision (d) Baseline (e) \aswnet{}.}
%\label{fig:results_more}
\end{figure*} 

==> rebuttal/defs.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\newif\ifdraft
\draftfalse
\drafttrue % <---- The way to switch between draft mode is to comment this


\definecolor{orange}{rgb}{1,0.5,0}
\definecolor{violet}{RGB}{70,0,170}
\definecolor{magenta}{RGB}{170,0,170}
\definecolor{dgreen}{RGB}{0,150,0}

% Strikethrough
\usepackage[normalem]{ulem}

\ifdraft
\newcommand{\PF}[1]{{\color{red}{\bf PF: #1}}}
\newcommand{\pf}[1]{{\color{red} #1}}
\newcommand{\PUW}[1]{{\color{blue}{\bf PUW: #1}}}
\newcommand{\puw}[1]{{\color{blue} #1}}
\newcommand{\MS}[1]{{\color{dgreen}{\bf MS: #1}}}
\newcommand{\ms}[1]{{\color{dgreen} #1}}
\newcommand{\PMJ}[1]{{\color{magenta}{\bf PMJ: #1}}}
\newcommand{\pmj}[1]{{\color{magenta} #1}}
\else
\newcommand{\PF}[1]{}
\newcommand{\pf}[1]{#1}
\newcommand{\PUW}[1]{}
\newcommand{\puw}[1]{#1}
\newcommand{\MS}[1]{}
\newcommand{\ms}[1]{#1}
\newcommand{\PMJ}[1]{}
\newcommand{\pmj}[1]{#1}
\fi

\newcommand{\comment}[1]{}
\newcommand{\parag}[1]{\vspace{-3mm}\paragraph{#1}}
\newcommand{\sparag}[1]{\vspace{-3mm}\subparagraph{#1}}
\renewcommand{\floatpagefraction}{.99}

% Graph
\newcommand{\gM}{\mathcal{M}}
\newcommand{\gE}{\mathcal{E}} 

% Matrices
\newcommand{\mA}{\mathbf{A}}
\newcommand{\mF}{\mathbf{F}}
\newcommand{\mG}{\mathbf{G}}
\newcommand{\mL}{\mathcal{L}}
\newcommand{\mS}{\mathcal{S}}
\newcommand{\mT}{\mathcal{T}}
\newcommand{\mM}{\mathbf{M}} 
\newcommand{\mP}{\mathbf{P}} 
\newcommand{\mU}{\mathbf{U}}   
\newcommand{\mV}{\mathbf{V}}  
\newcommand{\mW}{\mathbf{W}} 
\newcommand{\mX}{\mathbf{X}} 
\newcommand{\mY}{\mathbf{Y}} 
\newcommand{\mZ}{\mathbf{Z}}  

% feature vectors
\newcommand{\itf}{\textit{{f}}} 
\newcommand{\itg}{\textit{{g}}} 
\newcommand{\ith}{\textit{{h}}} 
\newcommand{\itv}{\textit{{v}}} 

% functions
\newcommand{\bif}{\textbf{\textit{f}}} 
\newcommand{\biG}{\textbf{\textit{g}}} 
\newcommand{\bih}{\textbf{\textit{g}}}  

% number sets
\newcommand{\real}{\mathbb{R}}
\newcommand{\X}{\mathcal{X}} 
\newcommand{\Z}{\mathcal{Z}} 
\newcommand{\V}{\mathcal{V}} 
\newcommand{\U}{\mathcal{U}} 

% vectors
\newcommand{\bv}[0]{\mathbf{v}}

% matrices
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bX}[0]{\mathbf{X}}
\newcommand{\bY}[0]{\mathbf{Y}}



\newcommand{\BASIC}[0]{\textbf{BASIC}}
\newcommand{\OURS}[0]{\textbf{OURS}}

\newcommand{\unet}[0]{\textbf{U-NET}} 
\newcommand{\vnet}[0]{\textbf{V-NET}}
\newcommand{\aswnet}[0]{\textbf{Weak-Net}}
\newcommand{\linknet}[0]{\textbf{LinkNet34}}
\newcommand{\resnet}[0]{\textbf{ResNet50}}
\newcommand{\resnetse}[0]{\textbf{ResNet50-SE}}
\newcommand{\dualtailnet}[0]{\textbf{DualTailNet}}
\newcommand{\unetpp}[0]{\textbf{U-Net++}}

\newcommand{\voxmeshplus}[0]{\textbf{Vox2Mesh+}}
\newcommand{\voxmesh}[0]{\textbf{Voxel2Mesh}}
\newcommand{\pixmesh}[0]{\textbf{Pixel2Mesh-3D}}
\newcommand{\pixelmesh}[0]{\textbf{Pixel2Mesh-3D}}
\newcommand{\pixelmeshpp}[0]{\textbf{Pixel2Mesh++}}

\newcommand{\fv}[0]{\textbf{x}}
\newcommand{\fy}[0]{\textbf{y}}
\newcommand{\ff}[0]{\textbf{f}}
\newcommand{\fm}[0]{\textbf{z}}





% Vectors:
\newcommand{\colvecTwo}[2]{\ensuremath{
		\begin{bmatrix}{#1}	\\	{#2}	\end{bmatrix}
}}
\newcommand{\colvec}[3]{\ensuremath{
		\begin{bmatrix}{#1}	\\	{#2}	\\	{#3} \end{bmatrix}
}}
\newcommand{\colvecFour}[4]{\ensuremath{
		\begin{bmatrix}{#1}	\\	{#2}	\\	{#3} \\	{#4}	\end{bmatrix}
}}

\newcommand{\rowvecTwo}[2]{\ensuremath{
		\begin{bmatrix}{#1}	&	{#2}	\end{bmatrix}
}}
\newcommand{\rowvec}[3]{\ensuremath{
		\begin{bmatrix}{#1} &	{#2}	&	{#3} \end{bmatrix}
}}
\newcommand{\rowvecFour}[4]{\ensuremath{
		\begin{bmatrix}{#1}	&	{#2}	&	{#3} &	{#4}	\end{bmatrix}
}}

% Transpose:
\newcommand{\tr}{^\intercal}

% Multi-row in matrices
\usepackage{multirow}

\DeclareMathOperator{\argmin}{\arg \min}



==> tab/results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
 

 
 \begin{table}[]
 		\centering
 	\caption{Comparative results}
 	\label{table:ablation_results}
 	\begin{tabular}{llll}
 		\hline
 		& Hippocampus    & Liver          & Synaptic Junction \\ \hline
 		Baseline & 71.2 $\pm$ 0.9 & 81.2 $\pm$ 0.8 & 68.2 $\pm$ 0.9    \\
 		\aswnet{}                 & 73.4 $\pm$ 0.8 & 83.1 $\pm$ 1.1 & 71.2 $\pm$ 1.2    \\
 	Full annotation & 79.3 $\pm$ 0.4 & 87.3 $\pm$ 0.3 &  76.2 $\pm$ 0.6                  \\ \hline
 	\end{tabular}
 \end{table}

==> tex/6_acknowledgment.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US
\section{Acknowledgments} This work was supported in part by a Swiss National Science Foundation grant. 


==> tex/7_check_list.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
	justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
	\item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
	\item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
	\item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}
	
	\item For all authors...
	\begin{enumerate}
		\item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
		\answerYes{}
		\item Did you describe the limitations of your work?
		\answerYes{See Sec.~\ref{sec:limitations}}
		\item Did you discuss any potential negative societal impacts of your work?
		\answerYes{See Sec.~\ref{sec:neg_img}}
		\item Have you read the ethics review guidelines and ensured that your paper conforms to them?
		\answerYes{}
	\end{enumerate}
	
	\item If you are including theoretical results...
	\begin{enumerate}
		\item Did you state the full set of assumptions of all theoretical results?
		\answerNA{}
		\item Did you include complete proofs of all theoretical results?
	    \answerNA{}
	\end{enumerate}
	
	\item If you ran experiments...
	\begin{enumerate}
		\item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
		\answerNo{The code will be published upon acceptance. Synaptic Junction Dataset will be made publicly available upon acceptance. The other two datasets are publicly available.}
		\item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
		\answerYes{See Supplementary Material}
		\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
		\answerNo{Only in Table~\ref{table:ablation_results}. For the rest of the experiment, we did not have necessary computational resources.}
		\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
		\answerYes{See Supplementary Material}
	\end{enumerate}
	
	\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
	\begin{enumerate}
		\item If your work uses existing assets, did you cite the creators?
		\answerNA{We used our own implementations}
		\item Did you mention the license of the assets?
		\answerNA{}
		\item Did you include any new assets either in the supplemental material or as a URL?
		\answerNA{}
		\item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
		\answerNA{Synaptic Junction Dataset will be made publicly available upon acceptance. The other two datasets are publicly available}
		\item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
		\answerNA{}
	\end{enumerate}
	
	\item If you used crowdsourcing or conducted research with human subjects...
	\begin{enumerate}
		\item Did you include the full text of instructions given to participants and screenshots, if applicable?
		\answerNA{}
		\item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
		\answerNA{}
		\item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
	   \answerNA{}
	\end{enumerate}
	
\end{enumerate}
